On the Computation of the Logarithm of the Modified Bessel Function of the Second Kind

The modified Bessel function of the second kind K$\nu$ appears in a wide variety of applied scientific fields. While its use is greatly facilitated by an implementation in most numerical libraries, overflow issues can be encountered especially for large value of $\nu$. After giving some necessary and sufficient conditions for their occurrences, this technical note shows that they can mostly be avoided by directly computing the logarithm of K$\nu$ thanks to a simple and stable forward recursion. A statistical examples based on the Gil-Pelaez inversion formula is given to illustrate the recursive method.

==> src/abstract.tex <==
The modified Bessel function of the second kind $K_\nu$ appears in a wide variety of applied scientific fields. While its use is greatly facilitated by an implementation in most numerical libraries, overflow issues can be encountered especially for large value of $\nu$. After giving some necessary and sufficient conditions for their occurrences, this technical note shows that they can mostly be avoided by directly computing the logarithm of $K_\nu$ thanks to a simple recurrence algorithm.

==> src/draft.tex <==
\pagebreak
\newpage
\section{Details to Be Removed}
%%%%%%%%%%%%%%%%%%
% Gamma function %
%%%%%%%%%%%%%%%%%%
\subsection{Gamma function}
Gamma function for integer:
\begin{equation}
 \displaystyle \Gamma (n)=(n-1)!   
\end{equation}

\citet{karatsuba2001asymptotic} bounds on Gamma function
\begin{equation}
    \label{eq:gamma_bound}
    \sqrt{\pi}\left({\frac{x}{e}}\right)^x
    \left({8x^3 + 4x^2 + x + \frac{1}{100}}\right)^{\frac16}
    <
    \Gamma(1+x)
    <
    \sqrt{\pi}\left({\frac{x}{e}}\right)^x
    \left({8x^3 + 4x^2 + x + \frac{1}{30}}\right)^{\frac16}
\end{equation}
\begin{eqnarray*}
    \sqrt{2\pi x}\left({\frac{x}{e}}\right)^x
    \left({1 + \frac{1}{2x} + \frac{1}{8x^2} + \frac{1}{800x^3}}\right)^{\frac16}
    &<
    x\Gamma(x)
    <&
    \sqrt{2\pi x}\left({\frac{x}{e}}\right)^x
    \left({1 + \frac{1}{2x} + \frac{1}{8x^2} + \frac{1}{240x^3}}\right)^{\frac16}
    \\%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \sqrt{\frac{2}{e}}\left({\frac{x}{e}}\right)^{x-\frac12}
    \left({1 + \frac{1}{2x} + \frac{1}{8x^2} + \frac{1}{800x^3}}\right)^{\frac16}
    &<
    \displaystyle\frac{\Gamma(x)}{\sqrt{\pi}}
    <&
    \sqrt{\frac{2}{e}}\left({\frac{x}{e}}\right)^{x-\frac12}
    \left({1 + \frac{1}{2x} + \frac{1}{8x^2} + \frac{1}{240x^3}}\right)^{\frac16}
\end{eqnarray*}
For $x\geq1$,
\begin{eqnarray*}
    \\%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \sqrt{\frac{2}{e}}\left({\frac{x}{e}}\right)^{x-\frac12}
    &<
    \displaystyle\frac{\Gamma(x)}{\sqrt{\pi}}
    <&
    \left({\frac{x}{e}}\right)^{x-\frac12}
    \\%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \left({
        \frac{2}{e}
    }\right)^{\frac1{2x-1}}
    \frac{x}{e}
    &<
    \left({
        \displaystyle\frac{\Gamma(x)}{\sqrt{\pi}}
    }\right)^{\frac1{x-\frac12}}
    <&
    \frac{x}{e}
    \\%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    2\left({
        \frac{2}{e}
    }\right)^{\frac1{2x-1}}
    \frac{x}{e}
    &<
    c_0=2\left({
        \displaystyle\frac{\Gamma(x)}{\sqrt{\pi}}
    }\right)^{\frac1{x-\frac12}}
    <&
    2\frac{x}{e}
\end{eqnarray*}


Then for $\nu\geq1$, 
\begin{equation}
    \label{eq:bound_b_1}
    b_1 \leq 
    \max\left\{
    \frac{2}{e}\nu,\ 
    \frac{\nu}{2}+\frac14    \right\}
\end{equation}


%%%%%%%%%%%%%%%%%%%
% Bessel Function %
%%%%%%%%%%%%%%%%%%%
\subsection{Bessel Function}
\begin{equation}
    K_{\frac12}(z)
    ={\sqrt {\frac {\pi }{2z}}}\cdot e^{-z}
\end{equation}



$K_\nu(z)$ has a rapid decay as $|z|$ grows~\citep{abramowitz1964handbook, watson1995treatise}, which may cause floating point underflow: 
\begin{equation}
    \label{eq:bessel_z_infty}
    K_\nu(z)
    \underset{|z|\to\infty}{\sim} 
    K_{\frac12}(z)=
    e^{-z}\sqrt{\frac{\pi}{2z}}.
\end{equation}
A non-asymptotic characterization was given for real values by~\citet{miller2001completely} who proved the complete monotonicity
of 
$
    z~\mapsto~z^{\min{\left(\frac12, \nu\right)}} e^z K_\nu(z)
$
for non-negative $\nu$.
\citet{yang2021monotonicity} proved the following inequalities bounds for for $z>0$ and $\nu\geq1$:
\begin{equation}
    \left({z+a_1}\right)^{\nu-\frac12}
    <
    \sqrt{\frac{2}{\pi}}z^\nu e^z K_\nu(z)
    <
    \left({z+b_1}\right)^{\nu-\frac12}
\end{equation}
with
\begin{equation*}
    a_1 = \min\left\{{
    c_0,\ \frac\nu2 + \frac14
    }\right\}
    \quad\textrm{and}\quad
    b_1 = \max\left\{{
    c_0,\ \frac\nu2 + \frac14
    }\right\}
\end{equation*}
where 
\begin{equation*}
    c_0 = 2\left({\frac{\Gamma(\nu)}{\sqrt\pi}}\right)^{\frac2{2\nu-1}}
\end{equation*}
They also proved that:
\begin{equation}
    \left({1+a_2z}\right)^{\nu-\frac12}
    <
    \frac{2}{\Gamma(\nu)}\left(\frac z2\right)^\nu e^z K_\nu(z)
    <
    \left({1+b_2z}\right)^{\nu-\frac12}
\end{equation}
with 
\begin{equation*}
    a_2 = \frac{1}{\max\left\{{
    c_0,\ \nu-\frac12
    }\right\}}
    \quad\textrm{and}\quad
    b_2 = \frac{1}{\min\left\{{
    c_0,\ \nu-\frac12
    }\right\}}
\end{equation*}

Deriving an upper bound:
\begin{eqnarray*}
    \displaystyle 
    \sqrt{\frac2\pi}z^\nu e^z K_\nu(z)
    &<&\displaystyle
    \left({z+b_1}\right)^{\nu-\frac12}
    %
    \\\displaystyle
    K_\nu(z)
    &<&\displaystyle
    \sqrt{\frac\pi2}z^{-\nu} e^{-z}
    \left({z+b_1}\right)^{\nu-\frac12}
    \\\displaystyle
    K_\nu(z)
    &<&\displaystyle
    \sqrt{\frac\pi{2z}} e^{-z}
    \left({1+\frac{b_1}{z}}\right)^{\nu-\frac12}
\end{eqnarray*}

\begin{equation}
    K_{\frac12}(z)\left({1+\frac{a_1}{z}}\right)^{\nu-\frac12}
    <
    K_\nu(z)
    <
    K_{\frac12}(z)\left({1+\frac{b_1}{z}}\right)^{\nu-\frac12}
\end{equation}

Using \eqref{eq:bound_b_1},
for $z\geq 
    \max\left\{
    \frac{2}{e}\nu,\ 
    \frac{\nu}{2}+\frac14    \right\}$, 

\begin{equation}
    K_\nu(z)
    <
    K_{\frac12}(z)\cdot 2^{\nu-\frac12} 
    =
     e^{-z}\sqrt{\frac{\pi}{z}}\cdot 2^{\nu-1}
\end{equation}

\begin{eqnarray*}
z &=& \frac12 W_0\left({\frac{\pi 2^{2\nu-1}}{L^2}}\right) 
\end{eqnarray*}

If $0 \leq\nu<\mu$ and $|\operatorname{ph}(z)| < \pi$, then
\begin{equation}
    |K_\nu(z)|< |K_\mu(z)|
\end{equation}

More recently, \citet{yang2021monotonicity} gave the following upper bound for $z>0$ and $\nu\geq1$:
\begin{equation}
    K_\nu(z)
    <
    \sqrt{\frac{\pi}{2z}} e^{-z} 
    \left({1+\frac{b}z}\right)^{\nu-\frac12}
\end{equation}
with
$\displaystyle
    b = \max\left\{{
    \ \frac\nu2 + \frac14,\ 
    2\left({\frac{\Gamma(\nu)}{\sqrt\pi}}\right)^{\frac2{2\nu-1}}
    }\right\}
$.
Noting, that based on~\citep{karatsuba2001asymptotic} upper bound on the Gamma function, 
$$
  2\left(\frac{\Gamma(\nu)}{\sqrt{\pi}}\right)^{\frac1{\nu-\frac12}} \leq 2\frac{\nu}{e}
$$
% \begin{eqnarray*}
%     \Gamma(\nu) &\leq& \sqrt{\pi}\left(\frac{\nu}{e}\right)^{\nu-\frac12}
%     \\
%     %
%     2\left(\frac{\Gamma(\nu)}{\sqrt{\pi}}\right)^{\frac1{\nu-\frac12}} &\leq& 2\frac{\nu}{e}
% \end{eqnarray*}
\begin{equation}
    \left({1+a_2z}\right)^{\nu-\frac12}
    <
    \frac{2}{\Gamma(\nu)}\left(\frac z2\right)^\nu e^z K_\nu(z)
    <
    \left({1+b_2z}\right)^{\nu-\frac12}
\end{equation}
with 
\begin{equation*}
    a_2 = \frac{1}{\max\left\{{
    c_0,\ \nu-\frac12
    }\right\}}
    \quad\textrm{and}\quad
    b_2 = \frac{1}{\min\left\{{
    c_0,\ \nu-\frac12
    }\right\}}
\end{equation*}

\begin{eqnarray*}
\frac{2}{\Gamma(\nu)}\left(\frac z2\right)^\nu e^z K_\nu(z)
&>& \left({1+a_2z}\right)^{\nu-\frac12}
\\
  K_\nu(z)
&>&
\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu
\left({1+a_2z}\right)^{\nu-\frac12}
\end{eqnarray*}

Since 
\begin{equation}
  c_0=2\left({
        \displaystyle\frac{\Gamma(x)}{\sqrt{\pi}}
    }\right)^{\frac1{x-\frac12}}
    <
    2\frac{x}{e}  
\end{equation},
for $\nu>\frac12/(1-2/e)$, $a2 = 1/(\nu-1/2)$.
  Then, 
  \begin{eqnarray*}
  K_\nu(z)
&>&
\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu
\left({1+\frac{z}{\nu-\frac12}}\right)^{\nu-\frac12}
\\
&>&
\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu
\\
&>&
\frac12\sqrt{\frac{2\pi}{e}}\left({\frac{\nu}{e}}\right)^{\nu-\frac12}
e^{-z}
\left(\frac 2z\right)^\nu
\\
&>&
\frac12e^{-z}
\sqrt{\frac{2\pi}{e}
\frac 2z}
\left({\frac{\nu}{e} \frac 2z}\right)^{\nu-\frac12}
\\
&>&
e^{-z}
\sqrt{\frac{\pi}{ez}}
\left({\frac{2(\nu-1/2)}{ez}}\right)^{\nu-\frac12}
\end{eqnarray*}

For
\begin{equation}
    \nu\geq
   \frac{1}{2} 
   + \frac{\log(P) +z - 0.5\log(\frac{\pi}{ez}) 
   }{W_0\left({
   \frac{2}{ez}
   \left({
   \log(P) +z - 0.5\log(\frac{\pi}{ez}
   }\right)
   }\right)} 
\end{equation}
$K_v(z)>P$


==> src/proof1.tex <==
\begin{proof}
Let $\nu$, $z$ and $B$ verify the hypotheses of proposition~\ref{prop:underflow_necessary}. According to Hoorfar and Hassani's bounds on the Lambert's function $W_0$~\cite{hoorfar2008inequalities} (theorem~2.7), since $x_0\geq e$, then: 
$2z \geq W_0(x_0)$.
%
$W_0$ being increasing, this leads to 
\begin{equation}
   \label{eq:1proof_underflow_necessary}
    B \geq  2^{\nu-\frac12}K_{\frac12}(z)
\end{equation}
%
With the previous bounds on $c_0$ (inequalities~\eqref{eq:bound_c0}), $b_1$ satisfies:
$$\displaystyle
    b_1 \leq 
    \max\left\{
    \frac{2}{e}\nu,\ 
    \frac{\nu}{2}+\frac14    \right\}
    \leq z
$$
% \begin{equation}
%     \label{eq:bound_b_1}
%     b_1 \leq 
%     \max\left\{
%     \frac{2}{e}\nu,\ 
%     \frac{\nu}{2}+\frac14    \right\}
%     \leq z
% \end{equation}
As a result, inequalities~\eqref{eq:1proof_underflow_necessary}
and~\eqref{eq:yang_bounds1} yield:
$$\displaystyle\quad
    B \geq   2^{\nu-\frac12}K_{\frac12}(z)
    \geq \left(1+\frac{b_1}{z}\right)^{\nu-\frac12}K_{\frac12}(z)
    \geq K_\nu(z)
$$
% \hfill\qedsymbol
\end{proof}

==> src/proof1_detailed.tex <==
\begin{proof} 
Let $\nu$, $z$ and $B$ verify the hypotheses of proposition~\ref{prop:underflow_necessary}. According to \citet{hoorfar2008inequalities}'s bounds on the Lambert's function $W_0$ (theorem~2.7), since $x_0\geq e$,
\begin{equation*}
    2z \geq W_0(x_0)
\end{equation*}
$W_0$ being increasing, 
\begin{eqnarray*}
    2z e^{2z} &\geq& \frac{2^{2\nu-1}\pi}{B^2}
    \\
    B^2 &\geq&  2^{2\nu-2}e^{-2z}\frac{\pi}{z} 
    \\
    B &\geq&  2^{\nu-1}e^{-z}\sqrt{\frac{\pi}{z}}
\end{eqnarray*}
\begin{equation}
   \label{eq:1proof_underflow_necessary}
    B \geq  2^{\nu-\frac12}K_{\frac12}(z)
\end{equation}

According to \citet{karatsuba2001asymptotic}, since $\nu>0$ the Gamma function verifies:
\begin{equation}
    \label{eq:gamma_bound}
    \left({8\nu^3 + 4\nu^2 + \nu + \frac{1}{100}}\right)^{\frac16}
    <
    \frac{\nu\Gamma(\nu)}{\sqrt{\pi}}
    \left({\frac{e}{\nu}}\right)^\nu
    <
    \left({8\nu^3 + 4\nu^2 + \nu + \frac{1}{30}}\right)^{\frac16}
\end{equation}
Then,
\begin{eqnarray*}
    \left({8 + \frac4\nu + \frac1{\nu}^2 + \frac{1}{100\nu^3}}\right)^{\frac16}
    &<\displaystyle
    \sqrt{e}
    \frac{\Gamma(\nu)}{\sqrt{\pi}}
    \left({\frac{e}{\nu}}\right)^{\nu-\frac12}
    <&
    \left({8 + \frac4\nu + \frac1{\nu}^2 + \frac{1}{30\nu^3}}\right)^{\frac16}
    \\
\end{eqnarray*}
Since $\nu\geq1$,
\begin{equation}
    \label{eq:gamma_bounds}
    \sqrt{\frac{2}{e}}
    <
    \frac{\Gamma(\nu)}{\sqrt{\pi}}
    \left({\frac{e}{\nu}}\right)^{\nu-\frac12}
    <
    1
\end{equation}
\begin{equation}
    \label{eq:bound_c0}
    2\frac\nu{e}
    \left({
        \frac{2}{e}
    }\right)^{\frac1{2\nu-1}}
    <
    c_0=2\left({
        \displaystyle\frac{\Gamma(\nu)}{\sqrt{\pi}}
    }\right)^{\frac1{\nu-\frac12}}
    <
    2\frac\nu{e}
\end{equation}

Hence, since $\nu\geq1$, 
\begin{equation*}
    \label{eq:bound_b_1}
    b_1 \leq 
    \max\left\{
    \frac{2}{e}\nu,\ 
    \frac{\nu}{2}+\frac14    \right\}
    \leq z
\end{equation*}
As a result, inequalities~\eqref{eq:1proof_underflow_necessary}
and~\eqref{eq:yang_bounds1} yield:
\begin{equation*}
    B \geq   2^{\nu-\frac12}K_{\frac12}(z)
    \geq \left(1+\frac{b_1}{x}\right)^{\nu-\frac12}K_{\frac12}(z)
    \geq K_\nu(z)
\end{equation*}

\end{proof}

==> src/proof3.tex <==

\begin{proof}
Since $a_2$ is defined in equation~\eqref{eq:def_ab2} is positive, inequality~\eqref{eq:yang_bounds2} yields:
\begin{equation}
\label{eq:start_proof_over}
K_\nu(z)>\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu    
\end{equation}

\noindent
The Gamma function can be bounded from below using Karatsuba's inequalities~\cite{karatsuba2001asymptotic}. Since $\nu>0$ the Gamma function verifies:
\begin{equation}
    \left({8\nu^3 + 4\nu^2 + \nu + \frac{1}{100}}\right)^{\frac16}
    <
    \frac{\nu\Gamma(\nu)}{\sqrt{\pi}}
    \left({\frac{e}{\nu}}\right)^\nu
    <
    \left({8\nu^3 + 4\nu^2 + \nu + \frac{1}{30}}\right)^{\frac16}
\end{equation}
Then for $\nu\geq1$,
\begin{equation}
    \label{eq:gamma_bounds}
    \sqrt{\frac{2}{e}}
    <
    \frac{\Gamma(\nu)}{\sqrt{\pi}}
    \left({\frac{e}{\nu}}\right)^{\nu-\frac12}
    <
    1
\end{equation}
Plugged into inequality~\eqref{eq:start_proof_over}, this gives:
\begin{equation}
 \label{eq:proof3_1}
K_\nu(z)
\quad>\quad
\frac12\sqrt{\frac{2\pi}{e}}\left({\frac{\nu}{e}}\right)^{\nu-\frac12}
e^{-z}
\left(\frac 2z\right)^\nu
\quad>\quad
e^{-z}
\sqrt{\frac{\pi}{ez}}
\left({\frac{2(\nu-1/2)}{ez}}\right)^{\nu-\frac12}
\end{equation}
%
% \begin{eqnarray}
%  \nonumber
% K_\nu(z)&>&
% \frac12\sqrt{\frac{2\pi}{e}}\left({\frac{\nu}{e}}\right)^{\nu-\frac12}
% e^{-z}
% \left(\frac 2z\right)^\nu
% % \\
% % &>&
% % \frac12e^{-z}
% % \sqrt{\frac{2\pi}{e}
% % \frac 2z}
% % \left({\frac{\nu}{e} \frac 2z}\right)^{\nu-\frac12}
%  \\\label{eq:proof3_1}
% K_\nu(z) &>&
% e^{-z}
% \sqrt{\frac{\pi}{ez}}
% \left({\frac{2(\nu-1/2)}{ez}}\right)^{\nu-\frac12}
% \end{eqnarray}
%

\noindent
Since $W_0(x) < x$ for all $x>-\frac1e$, the constraint $z>\frac{\pi}{B^2e}$ yields to:
\begin{equation*}
     \log(B) + z - \frac12\log(\frac{\pi}{ze}) > 0
\end{equation*}
% straight forward with W_0(0) = 0 + derivative < 1
\noindent
Then, inequality~\eqref{eq:overflow_necessary} leads to:
\begin{eqnarray}
%   \nu&\geq&\displaystyle
%     \frac12
%     +
%     \frac{\log(B) + z - \frac12\log(\frac{\pi}{ze})}{
%     W_0\left({\frac{2}{ze}
%     \left({
%     \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
%     }\right)
%     }
%     \\
%   \frac2{ze}(\nu-1/2)&\geq&\displaystyle  
%   \frac{\frac{2}{ze}
%     \left({
%     \log(B) + z - \frac12\log(\frac{\pi}{ze}}\right)}
%   {
%     W_0\left({\frac{2}{ze}
%     \left({
%     \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
%     }\right)
%     }
    %   \\
    \nonumber
      \frac2{ze}(\nu-1/2)&\geq&\displaystyle  
  \exp\left(
  {
    W_0\left({\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    }\right)
    }\right)
    % \\
    %   \log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    % W_0\left({\frac{2}{ze}
    % \left({
    % \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    % }\right)
        \\\nonumber
      \left({\frac2{ze}(\nu-1/2)}\right)\log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    \frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    % \\
    %   \left({\nu-1/2}\right)\log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    % \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)
    \\\label{eq:proof3_2}
      \left({\frac2{ze}(\nu-1/2)}\right)^{\left({\nu-1/2}\right)}
      &\geq&\displaystyle  
    B e^z \sqrt{\frac{ze}{\pi}}
\end{eqnarray}
Combining inequalities~\eqref{eq:proof3_1} and~\eqref{eq:proof3_2} proves proposition~\ref{prop:overflow_necessary}.
\hfill\qedsymbol
\end{proof}

==> src/proof3_detailed.tex <==

\begin{proof} \textbf{detailed}
Since $\nu\geq\frac{e}{2(e-2)}$, the upper bound~\eqref{eq:bound_c0} on $c_0$ leads to $$a_2 = (\nu-1/2)^{-1}$$ where $a_2$ is defined in equation~\eqref{eq:def_ab2}. Plugged into the inequality~\eqref{eq:yang_bounds2}, this yields:
 \begin{eqnarray*}
  K_\nu(z)
&>&
\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu
\left({1+\frac{z}{\nu-\frac12}}\right)^{\nu-\frac12}
\\
&>&
\frac{\Gamma(\nu)}2e^{-z}
\left(\frac 2z\right)^\nu
\\
&>&
\frac12\sqrt{\frac{2\pi}{e}}\left({\frac{\nu}{e}}\right)^{\nu-\frac12}
e^{-z}
\left(\frac 2z\right)^\nu
\quad \textrm{(from equation~\eqref{eq:gamma_bounds})}
\\
&>&
\frac12e^{-z}
\sqrt{\frac{2\pi}{e}
\frac 2z}
\left({\frac{\nu}{e} \frac 2z}\right)^{\nu-\frac12}
\\
&>&
e^{-z}
\sqrt{\frac{\pi}{ez}}
\left({\frac{2(\nu-1/2)}{ez}}\right)^{\nu-\frac12}
\end{eqnarray*}

\begin{eqnarray*}
  \nu&\geq&\displaystyle
    \frac12
    +
    \frac{\log(B) + z - \frac12\log(\frac{\pi}{ze})}{
    W_0\left({\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    }\right)
    }
    \\
  \frac2{ze}(\nu-1/2)&\geq&\displaystyle  
  \frac{\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log(\frac{\pi}{ze}}\right)}
  {
    W_0\left({\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    }\right)
    }
      \\
      \frac2{ze}(\nu-1/2)&\geq&\displaystyle  
  \exp\left(
  {
    W_0\left({\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    }\right)
    }\right)
    \\
      \log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    W_0\left({\frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    }\right)
        \\
      \left({\frac2{ze}(\nu-1/2)}\right)\log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    \frac{2}{ze}
    \left({
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)}\right)
    \\
      \left({\nu-1/2}\right)\log\left({\frac2{ze}(\nu-1/2)}\right)&\geq&\displaystyle  
    \log(B) + z - \frac12\log\left({\frac{\pi}{ze}}\right)
    \\
      \left({\frac2{ze}(\nu-1/2)}\right)^{\left({\nu-1/2}\right)}
      &\geq&\displaystyle  
    B e^z \sqrt{\frac{ze}{\pi}}
\end{eqnarray*}

\end{proof}

==> src/proof4.tex <==
\begin{proof}
Bounds on $c_0$ can be directly obtained from inequality~\eqref{eq:gamma_bounds}:
\begin{equation}
    \label{eq:bound_c0}
    2\frac\nu{e}
    \left({
        \frac{2}{e}
    }\right)^{\frac1{2\nu-1}}
    <
    c_0=2\left({
        \displaystyle\frac{\Gamma(\nu)}{\sqrt{\pi}}
    }\right)^{\frac1{\nu-\frac12}}
    <
    2\frac\nu{e}
\end{equation}
%
According to inequality~\eqref{eq:yang_bounds1},  
%for $\nu\geq\displaystyle \frac{e}{2(e-2)}$,
for $\nu\geq\displaystyle \frac{e}{2(4-e)}$,
\begin{eqnarray}
    \nonumber
    K_\nu(z) &<& K_{\frac12}(z) \left({ 1+ \frac{2\nu}{ze}
    }\right)^{(\nu-\frac12)}
    =
    \left({ 1+ \frac{2\nu}{ze}}\right)^{(\nu+\frac{ze}{2})}
    \left({ 1+ \frac{2\nu}{ze}}\right)^{-(\frac{ze}{2}+\frac12)} K_{\frac12}(z)
    \\
    \label{eq:overflow_sufficient_proof}
    K_\nu(z)  &< &
    \left({\frac{2}{ze}\left(\nu + \frac{ze}{2}\right)}\right)^{(\nu+\frac{ze}{2})}
    \left({ 1+ \frac{2}{ze}}\right)^{-(\frac{ze}{2}+\frac12)} K_{\frac12}(z)
    \quad\quad\textrm{(since $\nu\geq1$)}
\end{eqnarray}
%
%
Since by definition, $\nu$ satisfies inequality~\eqref{eq:overflow_sufficient}, 
\begin{eqnarray*}
    \frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) 
    &\leq& \frac{\frac{2}{ze}\log x_0}{W_0\left(\frac{2}{ze}\log x_0\right)} = 
    \exp\left[{W_0\left(\frac{2}{ze}\log x_0\right)}\right]
    % \\
    % \log \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)
    % &\leq&
    % W_0\left(\frac{2}{ze}\log x_0\right)
    % \\
    % \left({\nu + \frac{ze}{2}}\right)\log \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)
    % &\leq&
    % \log x_0
    \\
    \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)^{\left({\nu + \frac{ze}{2}}\right)}
    &\leq&
    x_0 = \frac{B}{K_{\frac12}(z)}\left({1 + \frac{2\nu}{ze}}\right)^{\frac{1+ze}{2}}
\end{eqnarray*}
Hence, using inequality~\eqref{eq:overflow_sufficient_proof}, $K_\nu(z) < B$.
% \hfill\qedsymbol
\end{proof}

==> src/proof4_detailed.tex <==
\begin{proof}

According to inequality~\eqref{eq:yang_bounds1}, 
for $\nu\geq\displaystyle \frac{e}{2(e-2)}$
\begin{eqnarray*}
    K_\nu(z) &<& K_{\frac12}(z) \left({ 1+ \frac{2\nu}{ze}
    }\right)^{(\nu-\frac12)}
    \\
    &<&
    \left({ 1+ \frac{2\nu}{ze}}\right)^{(\nu+\frac{ze}{2})}
    \left({ 1+ \frac{2\nu}{ze}}\right)^{-(\frac{ze}{2}+\frac12)} K_{\frac12}(z)
\end{eqnarray*}
\begin{equation}
    \label{eq:overflow_sufficient_proof}
    K_\nu(z) < 
    \left({\frac{2}{ze}\left(\nu + \frac{ze}{2}\right)}\right)^{(\nu+\frac{ze}{2})}
    \left({ 1+ \frac{2}{ze}}\right)^{-(\frac{ze}{2}+\frac12)} K_{\frac12}(z)
    \quad\textrm{(since $\nu\geq1$)}
\end{equation}


$\nu$ verifies:
\begin{eqnarray*}
    \frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) 
    &\leq& \frac{\frac{2}{ze}\log x_0}{W_0\left(\frac{2}{ze}\log x_0\right)} = 
    \exp\left[{W_0\left(\frac{2}{ze}\log x_0\right)}\right]
    \\
    \log \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)
    &\leq&
    W_0\left(\frac{2}{ze}\log x_0\right)
    \\
    \left({\nu + \frac{ze}{2}}\right)\log \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)
    &\leq&
    \log x_0
    \\
    \left({\nu + \frac{ze}{2}}\right)\log \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)
    &\leq&
    \log x_0
    \\
    \left({\frac{2}{ze}\left({\nu + \frac{ze}{2}}\right) }\right)^{\left({\nu + \frac{ze}{2}}\right)}
    &\leq&
    x_0 = \frac{B}{K_{\frac12}(z)}\left({1 + \frac{2}{ze}}\right)^{\frac{1+ze}{2}}
\end{eqnarray*}
Hence, using inequality~\eqref{eq:overflow_sufficient_proof}, $K_\nu(z) < B$.
\end{proof}


\begin{proof}
According to~\eqref{eq:bound_c0}, 
\begin{equation*}
    c_0 <2\frac{\nu}{e}
\end{equation*}
Hence for $\nu\geq\displaystyle \frac{e}{2(e-2)}$, $b_2= 1/c_0$.
Therefore, based on inequalities~\eqref{eq:yang_bounds2}, for $\nu\geq\displaystyle \frac{e}{2(e-2)}$,
\begin{eqnarray*}
K_\nu(z)
&\leq &\displaystyle
    \frac{\Gamma(\nu)}{2}\left({\frac{2}{z}}\right)^{\nu}e^{-z}
    \left({1+\frac{z}{c_0}}\right)^{\nu-\frac12}
\\&\leq &\displaystyle
\Gamma(\nu)
\sqrt{\frac{1}{2z}}
\left({\frac{2}{z}}\right)^{\nu-\frac12}e^{-z}
    \left(\frac{z}{c_0}\right)^{\nu-\frac12}\left({1+\frac{c_0}{z}}\right)^{\nu-\frac12}
\\&\leq &\displaystyle
e^{-z}
\sqrt{\frac{\pi}{2z}}
    \left({1+\frac{c_0}{z}}\right)^{\nu-\frac12}
    \quad\textrm{(from equation~\eqref{eq:def_c0}})
\\&\leq &\displaystyle
K_{\frac12}(z)
    \left({1+\frac{2\nu}{ze}}\right)^{\nu-\frac12}
    \quad\textrm{(from equation~\eqref{eq:bound_c0}})
\end{eqnarray*}

\end{proof}

